Polyhedral Discretizations for Elliptic PDEs

We study the use of polyhedral discretizations for the solution of heat diffusion and elastodynamic problems in computer graphics. Polyhedral meshes are more natural for certain applications than pure triangular or quadrilateral meshes, which thus received significant interest as an alternative representation. We consider finite element methods using barycentric coordinates as basis functions and the modern virtual finite element approach. We evaluate them on a suite of classical graphics problems to understand their benefits and limitations compared to standard techniques on simplicial discretizations. Our analysis provides recommendations and a benchmark for developing polyhedral meshing techniques and corresponding analysis techniques.

==> 43-meshing.tex <==
\section{Meshing}\label{app:meshing}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Polygonal Meshing %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Polygonal and Polyhedral Mesh Generation}
\label{sec:Polygonal-Polyhedral-Mesh-Generation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Voronoi %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Voronoi}
In our experiments, we generate four Voronoi polygonal meshes using PolyMesher~\cite{PolyMesher} for each domain, with the CVT iteration number set as 1, 5, 10, and 20.

In 3D, Voro++ \cite{Voro++} provides three distributions of points: (1) Random sampling (similar to PolyMesher \cite{PolyMesher} with one iteration); (2) Poisson sampling with $1/n_P$ with $n_P$ the number of points; and (3). Body-Centered Lattice (BCL) sampling point distribution (similar to PolyMesher \cite{PolyMesher} with 20 iterations).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Displacement %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Displacement}
Displacement tessellations of 2D domains use several displacement functions to change the distribution of vertices from regularly structured meshes~\cite{Displacement-Polygon-Meshing-1,Displacement-Polygon-Meshing-2}. In our experiments, we use Veamy \cite{Veamy}, a software that collects commonly used displacement functions, including five functions for the distribution, (1) constant distribution, (2) uniform distribution, (3) altered distribution, (4) displaced distribution, and (5) random noise distribution along both the $x$ and $y$ axis.

Displacement meshes can be naturally extended to 3D, and \cite{Polyheral-quality-indicator} provides three kinds of displaced grids with different point distribution (Figure \ref{fig:polyhedra_displace}): (1) Uniform; (2) Anisotropic (the distribution is fixed along two axes and incrementally enlarged along the other axis); and (3) Parallel (the points are first uniformly sampled and then randomly moved to another inner plane which is parallel to the original plane. For example, the points sharing the same $x$ coordinate are randomly changed with $x$ value by the same quantity, and the same operation iterates to the $y$ and $z$ coordinates). After we generate the initial displaced grid, we obtain the polyhedral meshes by tetrahedralizing every cell and randomly aggregate $20\%$ of the elements to generate possibly non-convex polyhedral elements.

\begin{figure}
     \centering\footnotesize
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \includegraphics[width=.33\linewidth]{img/mesh/poly/para/hex-uniform-0}\hfill
     \includegraphics[width=.33\linewidth]{img/mesh/poly/para/hex-anisotropic-0}\hfill
     \includegraphics[width=.33\linewidth]{img/mesh/poly/para/hex-parallel-0}\par
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \parbox{.33\linewidth}{\centering Uniform (HP3D1)}\hfill
     \parbox{.33\linewidth}{\centering Anisotropic (HP3D2)}\hfill
     \parbox{.33\linewidth}{\centering Parallel (HP3D3)}
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \caption{Displacement polyhedral meshes generated by displacing a grid.}
     \label{fig:polyhedra_displace}
 \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Tiled %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Tiled}
Tiled polygonal meshing generates challenging meshes since most Voronoi and Displacement meshing produces mostly convex polygonal tessellations.
In our experiments, we use a similar approach as \cite{VEM-quality-benchmark}, in which we generate one concave-shaped polygon inside each element of structured quadrilateral meshes and then we perform a constrained Delaunay triangulation %\cite{Delaunay-Triangulation}
to fill the empty space. We use similar settings as in \cite{VEM-quality-benchmark} to generate five concave polygonal shapes (star-shaped, Z-shaped, U-shaped, maze-shaped, and comb-shaped) for each domain.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Simplicial Meshing %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Simplicial Mesh Generation}\label{subsec:Tri-Tet-Meshing}
To generate a fair dataset, we design several methods to ``convert'' our polygonal meshes into simplicial ones. Every approach strives to maintain the same number of vertices.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Dual %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Dual}
For the specific case of Voronoi meshes, the easiest triangulation method consists of using the dual to obtain a Delaunay mesh. In 3D, we use \cite{Polyheral-quality-indicator} to obtain the dual tetrahedral meshes.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Triangulation %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Triangulation}
Another method consists of triangulating the inside of each polygonal cell. In our experiment, we use four triangulation methods: (1) Ear Clip \cite{mapbox-earclip} using Mapbox; (2) insert a random point in each polygon cell and connect it with the boundary; (3) Constraint Delaunay Triangulation using~\cite{Triangle} with no additional Stainer points; and (4) Conforming Delaunay Triangulation using~\cite{Triangle}. We note that methods 1 and 2 work only with Voronoi and displacement meshes as the cells are convex.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Tetrahedralization %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Tetrahedralization}
\cite{Polyheral-quality-indicator} provides a method to tetrahedralize each polyhedral cell by iteratively splitting a polyhedral element with a diagonal plane until the left element is a tetrahedron.

==> 98-figures.tex <==

 \begin{figure}
     \centering\footnotesize
     \parbox{.02\linewidth}{~}\hfill\hfill
     \parbox{.32\linewidth}{\centering LEP-BE}\hfill
     \parbox{.32\linewidth}{\centering PS\#1-US}\hfill
     \parbox{.32\linewidth}{\centering PS\#2-SC}\par
     \parbox{.02\linewidth}{\rotatebox{90}{\centering Direct Solver}}\hfill\hfill
     \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/direct/1D_ranking/LEP-BE_L2_time}}\hfill
     \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/direct/1D_ranking/PS1-US_L2_time}}\hfill
     \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/direct/1D_ranking/PS2-SC_L2_time}}\par
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \parbox{.02\linewidth}{\rotatebox{90}{\centering Iterative Solver}}\hfill\hfill
     \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/pcg/1D_ranking/LEP-BE_L2_time}}\hfill
     \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/pcg/1D_ranking/PS1-US_L2_time}}\hfill
     \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/pcg/1D_ranking/PS2-SC_L2_time}}\par
     \includegraphics[width=\linewidth]{img/results/legend/1D_ranking}\par
     \caption{Comparison of solving with direct solvers and iterative solvers. The $x$-axis shows the $L_2$ error while the $y$-axis shows the time in seconds.}
     \label{fig:compare_solver}
 \end{figure}

  \begin{figure}
     \centering\footnotesize
     \parbox{.02\linewidth}{~}\hfill\hfill
     \parbox{.32\linewidth}{\centering $10^{-2}$}\hfill
     \parbox{.32\linewidth}{\centering $10^{-3}$}\hfill
     \parbox{.32\linewidth}{\centering $10^{-4}$}\par
     \parbox{.02\linewidth}{\rotatebox{90}{\centering Direct Solver}}\hfill\hfill
     \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results_new/VEMLab/direct/1D_all/PS1-SC_L2_norm1}}\hfill
     \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results_new/VEMLab/direct/1D_all/PS1-SC_L2_norm2}}\hfill
     \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results_new/VEMLab/direct/1D_all/PS1-SC_L2_norm3}}\par
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \parbox{.02\linewidth}{\rotatebox{90}{\centering Iterative Solver}}\hfill\hfill
     \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results_new/VEMLab/pcg/1D_all/PS1-SC_L2_norm1}}\hfill
     \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results_new/VEMLab/pcg/1D_all/PS1-SC_L2_norm2}}\hfill
     \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results_new/VEMLab/pcg/1D_all/PS1-SC_L2_norm3}}\par
     \includegraphics[width=0.8\linewidth]{img/results_new/legend/1D_all_legend}\par
     \caption{Comparison of PS1-SC solving time at 3 error levels with direct solvers and iterative solvers.}
     \label{fig:compare_solver}
 \end{figure}


\begin{figure}
    \centering\footnotesize
    \parbox{.02\linewidth}{~}\hfill\hfill
    \parbox{.32\linewidth}{\centering PS\#1-SC}\hfill
    % \parbox{.32\linewidth}{\centering LEP-BE}\hfill
    \parbox{.32\linewidth}{\centering PS\#3-UD}\hfill
    % \parbox{.32\linewidth}{\centering LEB-PH}\par
    \parbox{.32\linewidth}{\centering PB-LS}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \parbox{.02\linewidth}{\rotatebox{90}{\centering Direct Solver}}\hfill\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/direct/poly_vs_simplicial/voro/PS1-SC_L2_time}}\hfill
    % \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/direct/poly_vs_simplicial/voro/LEP-BE_L2_time}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/direct/poly_vs_simplicial/voro/PS3-UD_L2_time}}\hfill
    % \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/direct/poly_vs_simplicial/voro/LEB-PH_L2_time}}\par
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/direct/poly_vs_simplicial/voro/PB-LS_L2_time}}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \parbox{.02\linewidth}{\rotatebox{90}{\centering Iterative Solver}}\hfill\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/pcg/poly_vs_simplicial/voro/PS1-SC_L2_time}}\hfill
    % \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/pcg/poly_vs_simplicial/voro/LEP-BE_L2_time}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/pcg/poly_vs_simplicial/voro/PS3-UD_L2_time}}\hfill
    % \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/pcg/poly_vs_simplicial/voro/LEB-PH_L2_time}}\par
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/pcg/poly_vs_simplicial/voro/PB-LS_L2_time}}\par
    \includegraphics[width=\linewidth]{img/results/legend/poly_vs_simplicial_voro}\par
    \caption{Solving time (s) versus $L_2$ error for VP4 to its corresponding dual and four triangulated meshes.}
    \label{fig:compare_poly_vs_simplicial_voro}
\end{figure}


\begin{figure}
    \centering\footnotesize
    \parbox{.02\linewidth}{~}\hfill\hfill
    \parbox{.32\linewidth}{\centering PS\#1-SC}\hfill
    % \parbox{.32\linewidth}{\centering LEP-BE}\hfill
    \parbox{.32\linewidth}{\centering PS\#3-UD}\hfill
    % \parbox{.32\linewidth}{\centering LEB-PH}\par
    \parbox{.32\linewidth}{\centering PB-LS}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \parbox{.02\linewidth}{\rotatebox{90}{\centering Direct Solver}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/direct/poly_vs_simplicial/para/PS1-SC_L2_time}}\hfill
    % \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/direct/poly_vs_simplicial/para/LEP-BE_L2_time}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/direct/poly_vs_simplicial/para/PS3-UD_L2_time}}\hfill
    % \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/direct/poly_vs_simplicial/para/LEB-PH_L2_time}}\par
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/direct/poly_vs_simplicial/para/PB-LS_L2_time}}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \parbox{.02\linewidth}{\rotatebox{90}{\centering Iterative Solver}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/pcg/poly_vs_simplicial/para/PS1-SC_L2_time}}\hfill
    % \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/pcg/poly_vs_simplicial/para/LEP-BE_L2_time}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/pcg/poly_vs_simplicial/para/PS3-UD_L2_time}}\hfill
    % \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/pcg/poly_vs_simplicial/para/LEB-PH_L2_time}}\par
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/pcg/poly_vs_simplicial/para/PB-LS_L2_time}}\par
    \includegraphics[width=\linewidth]{img/results/legend/poly_vs_simplicial_para}\par
    \caption{Solving time (s) versus $L_2$ error for DP3 to its four triangulated meshes.}
    \label{fig:compare_poly_vs_simplicial_displace}
\end{figure}


\begin{figure}
    \centering\footnotesize
     \parbox{.02\linewidth}{~}\hfill
     \parbox{.32\linewidth}{\centering PS\#1-US}\hfill
     \parbox{.32\linewidth}{\centering PS\#1-SC}\hfill
     \parbox{.32\linewidth}{\centering PS\#2-US}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \parbox{.02\linewidth}{\rotatebox{90}{\centering DT}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/PolyFEM/direct/higher_order/voro_dual/PS1-US_L2_time}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/PolyFEM/direct/higher_order/voro_dual/PS1-SC_L2_time}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/PolyFEM/direct/higher_order/voro_dual/PS2-US_L2_time}}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \includegraphics[width=\linewidth]{img/results/legend/higher_order_voro_dual}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \parbox{.02\linewidth}{\rotatebox{90}{\centering VP4-PT}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/PolyFEM/direct/higher_order/voro_tri/PS1-US_L2_time}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/PolyFEM/direct/higher_order/voro_tri/PS1-SC_L2_time}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/PolyFEM/direct/higher_order/voro_tri/PS2-US_L2_time}}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \includegraphics[width=\linewidth]{img/results/legend/higher_order_voro_tri}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \parbox{.02\linewidth}{\rotatebox{90}{\centering DP-PT}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/PolyFEM/direct/higher_order/para_tri/PS1-US_L2_time}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/PolyFEM/direct/higher_order/para_tri/PS1-SC_L2_time}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/PolyFEM/direct/higher_order/para_tri/PS2-US_L2_time}}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \includegraphics[width=\linewidth]{img/results/legend/higher_order_para_tri}\par
    \caption{Comparison (time versus error) of linear FEM and higher-order FEM on triangular meshes.}
    \label{fig:high-order}
\end{figure}


\begin{figure}
    \centering\footnotesize
     \parbox{.02\linewidth}{~}\hfill
     \parbox{.32\linewidth}{\centering PS\#1-US}\hfill
     \parbox{.32\linewidth}{\centering PS\#1-SC}\hfill
     \parbox{.32\linewidth}{\centering PS\#2-SC}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \parbox{.02\linewidth}{\rotatebox{90}{\centering VP and DT}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/PolyFEM/direct/Meanvalue/voro_vs_dual/PS1-US_L2_time}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/PolyFEM/direct/Meanvalue/voro_vs_dual/PS1-SC_L2_time}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/PolyFEM/direct/Meanvalue/voro_vs_dual/PS2-SC_L2_time}}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \includegraphics[width=\linewidth]{img/results/legend/barycentric_tri_voro_dual}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \parbox{.02\linewidth}{\rotatebox{90}{\centering DP and PT}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/PolyFEM/direct/Meanvalue/para_vs_tri/PS1-US_L2_time}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/PolyFEM/direct/Meanvalue/para_vs_tri/PS1-SC_L2_time}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/PolyFEM/direct/Meanvalue/para_vs_tri/PS2-SC_L2_time}}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \includegraphics[width=\linewidth]{img/results/legend/barycentric_tri_para_tri}\par
    \caption{Comparison of barycentric FEM on polygon meshes and FEM on triangular meshes.}
    \label{fig:bary-vem}
\end{figure}

\begin{figure}
    \centering\footnotesize
    % \includegraphics[width=1\linewidth]{img/compare_VEM_stabilization}
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \parbox{.02\linewidth}{~}\hfill
    \parbox{.32\linewidth}{\centering Gain et al.}\hfill
    \parbox{.32\linewidth}{\centering Diagonal Recipe}\hfill
    \parbox{.32\linewidth}{\centering modified Diagonal Recipe}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \parbox{.02\linewidth}{\rotatebox{90}{\centering LEP-BE}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab_stable1/direct/LEP-BE_L2_time}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab_stable2/direct/LEP-BE_L2_time}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/direct/LEP-BE_L2_time}}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \parbox{.02\linewidth}{\rotatebox{90}{\centering LEB-PH}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab_stable1/direct/LEB-PH_L2_time}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab_stable2/direct/LEB-PH_L2_time}}\hfill % To be filled up
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/direct/LEB-PH_L2_time}}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \includegraphics[width=\linewidth]{img/results/legend/plot_all}\par
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caption{Comparison of different stabilization mechanisms of VEM on Linear Elasticity Problems.}
    \label{fig:compare_VEM_stabilization}
\end{figure}

\begin{figure}
    \centering\footnotesize
    \parbox{.499\linewidth}{\centering
    \parbox{.02\linewidth}{~}\hfill\hfill
    \parbox{.48\linewidth}{\centering PS\#2-US}\hfill
    \parbox{.48\linewidth}{\centering 3D}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \parbox{.02\linewidth}{\rotatebox{90}{\centering Direct Solver}}\hfill\hfill
    \parbox{.48\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/direct/PS2-US_L2_time}}\hfill
    \parbox{.48\linewidth}{\includegraphics[width=\linewidth]{img/results/3D/direct/3D_L2}}\par
    }\hfill
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \parbox{.499\linewidth}{\centering
    \parbox{.02\linewidth}{~}\hfill\hfill
    \parbox{.48\linewidth}{\centering PS\#2-US}\hfill
    \parbox{.48\linewidth}{\centering 3D}\par
    \parbox{.02\linewidth}{\rotatebox{90}{\centering Iterative Solver}}\hfill\hfill
    \parbox{.48\linewidth}{\includegraphics[width=\linewidth]{img/results/VEMLab/pcg/PS2-US_L2_time}}\hfill
    \parbox{.48\linewidth}{\includegraphics[width=\linewidth]{img/results/3D/pcg/3D_L2}}\par}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \parbox{.02\linewidth}{\rotatebox{90}{\centering PS\#2-US}}\hfill\hfill
    \parbox{.96\linewidth}{\includegraphics[width=\linewidth]{img/results/legend/plot_all}}\par
    \parbox{.02\linewidth}{\rotatebox{90}{\centering 3D}}\hfill\hfill
    \parbox{.96\linewidth}{\includegraphics[width=\linewidth]{img/results/legend/3D}}\par
    \caption{Comparison of 2D domain and 3D domain on Poisson Problems.}
    \label{fig:compare_2d_vs_3d}
\end{figure}

\begin{figure}
    \centering\footnotesize
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \parbox{.02\linewidth}{~}\hfill
    \parbox{.32\linewidth}{\centering 3D Poisson 1}\hfill
    \parbox{.32\linewidth}{\centering 3D Poisson 2}\hfill
    \parbox{.32\linewidth}{\centering 3D Poisson 3}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \parbox{.02\linewidth}{\rotatebox{90}{\centering Direct Solver}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results_new/3D/direct/pde1_3D_L2}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results_new/3D/direct/pde2_3D_L2}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results_new/3D/direct/pde3_3D_L2}}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \parbox{.02\linewidth}{\rotatebox{90}{\centering Iterative Solver}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results_new/3D/pcg/pde1_3D_L2}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results_new/3D/pcg/pde2_3D_L2}}\hfill
    \parbox{.32\linewidth}{\includegraphics[width=\linewidth]{img/results_new/3D/pcg/pde3_3D_L2}}\par
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \includegraphics[width=\linewidth]{img/results/legend/3D}\par
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caption{Comparison of 3 different 3D Poisson problem on cubes.}
    \label{fig:3D_poisson}
\end{figure}
